Extinction time of stochastic SIRS models with small initial size of the infected population

The stochastic SIRS model is a continuous-time Markov chain modelling the spread of infectious diseases with temporary immunity, in a homogeneously-mixing population of fixed size $N$. We study the scaling behaviour of the extinction time of stochastic SIRS models as $N$ tends to infinity. When the initial size of infected population is small, we obtain the closed-form expression of the asymptotic distribution of this extinction time, and compare it with the data from Monte Carlo simulation.

==> images/11/readme.tex <==
naming system of figure folder:
cdf.eps is the old version
toggle{
case11: PARA-l(1+0.5)g(0+0.16667)I(0.25)R(0.5)_neg
case11plus: PARA-l(1+0.5)g(0+0.16667)I(0.25)R(0.5)

the following are unused examples:
\twobytwofig{
Case 2.1 (b: $1-\lambda_o\to 0$)
\begin{align*}
    & N = 10^4,10^6,\cdots,10^{12},\\
    & 1-\lambda_o = N^{-1/3}, \, \gamma_o = N^{-5/12},\\
    & I_0 = 50,\, R_0 = 0.7N.
\end{align*}
%Note: the speed of convergence is slower if $\gamma_o$ tends to $0$ slower.
}
{./Chapter6/case21b/logpath.eps}{./Chapter6/case21b/pdf.eps}
{./Chapter6/case21b/cdf.eps}
{Sample path ($\log_{N}$), probability density and cumulative density of Case 2.1}{fig:case21b}


\twobytwofig{
Case 2.2 (b: $I_0(1-\lambda_o)\to 0$)
\begin{align*}
    & N = 10^4,10^6,\cdots,10^{12},\\
    & 1-\lambda_o = N^{-1/4}, \, \gamma_o = N^{-3/4},\\
    & I_0 = N^{1/5},\, R_0 = 0.4N.
\end{align*}
We set $n_c=250$.
}
{./Chapter6/case22e/logpath.eps}{./Chapter6/case22e/pdf.eps}
{./Chapter6/case22e/cdf.eps}
{Sample path ($\log_{N}$), probability density and cumulative density of Case 2.2}{fig:case22e}

\twobytwofig{
Case 2.2 (c: $I_0(1-\lambda_o)\to \infty$)
\begin{align*}
    & N = 10^4,10^6,\cdots,10^{12},\\
    & 1-\lambda_o = N^{-1/7}, \, \gamma_o = N^{-1/4},\\
    & I_0 = N^{1/5},\, R_0 = 0.7N.
\end{align*}
}
{./Chapter6/case22f/logpath.eps}{./Chapter6/case22f/pdf.eps}
{./Chapter6/case22f/cdf.eps}
{Sample path ($\log_{N}$), probability density and cumulative density of Case 2.2}{fig:case22f}





}

==> images/graph_parameter.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
        xmin=0, xmax=1.3,
        ymin=0, ymax=1.3,
        axis lines=middle,
        x label style={at={(axis description cs:2,0)}},
        y label style={at={(axis description cs:-0.2,2)}},
        xlabel = $-\log_N(1-\lambda_o)$, ylabel = $-\log_N(\gamma_o)$,
        ytick={0,1, 1.2},
        yticklabels={0,1,$\infty$},
        xtick={0,0.5,1,1.2},
        xticklabels={0,$1/2$,1, $\infty$},
      ]  
       \path[name path=xaxis] (\pgfkeysvalueof{/pgfplots/xmin}, 0) -- (\pgfkeysvalueof{/pgfplots/xmax},0);
       %\addplot [mark=none, dash pattern= on 3pt off 1pt] coordinates {(0.3333, 0) (0.3333, 0.3333)};
       %\addplot [mark=none, dash pattern= on 3pt off 1pt, name path= A] coordinates {(0, 0.3333) (0.3333, 0.3333)};
       %%
       %\addplot [ultra thick,mark=none, name path= A] coordinates {(0, 0) (0, 1)};
        \addplot[samples=100, domain=0:1, name path=B,dash pattern= on 3pt off 1pt] {1-2*x} node[above,pos=1] {$-\polyorder{1-\lambda_o} = \frac{1+\polyorder{\gamma_o}}{2}$}; 
        
        % \addplot[gray, pattern=north east lines] fill between[of=A and xaxis, soft clip={domain=0:0.3333}];
         \addplot[gray, pattern=vertical lines] fill between[of=B and xaxis, soft clip={domain=0:0.5}];
   \end{axis}
\end{tikzpicture}
